FedSwitch: Federated Region Classification From Wireless Channel Measurements

Wireless Internet-of-Things (IoT) networks can leverage locally observed channel state information (CSI) at base-stations (BSs) to perform region classification, i.e., infer the region of origin of a transmitter (TX), thereby enabling channel-based authentication. However, centralizing these measurements incurs substantial communication overhead and requires sharing location-dependent radio fingerprints. To address these difficulties, we propose an edge-native federated learning (FL) framework where BSs collaboratively train a shared classifier via a parameter server (PS) without exposing raw data, thereby supporting physical-layer security tasks like spoofing detection. To overcome the statistical heterogeneity arising from diverse BS locations and propagation conditions, we introduce FedSwitch, a personalized FL algorithm that automatically transitions edge nodes from collaborative training to local fine-tuning upon loss stagnation. We provide theoretical convergence guarantees for the proposed collaborative training phase and derive analytical bounds linking classification errors to statistical discrepancies. Extensive evaluations on synthetic channel measurements demonstrate that FedSwitch significantly improves region-classification accuracy over standard FL baselines.

==> plot_learning_curves.tex <==
\usetikzlibrary{intersections}
\usepgfplotslibrary{fillbetween}

\begin{tikzpicture}
\begin{axis}[
    width=\linewidth,
    height=0.6\linewidth,
    xlabel={Epochs},
    ylabel={Accuracy \%},
    grid=both,
    legend style={
        at={(0.98,0.02)},
        anchor=south east,
        font=\scriptsize,
        inner sep=2pt,
        row sep=1pt,
        column sep=2pt   % space between columns
    },
    legend columns=2,
    legend cell align={left}
]

%----- FED AVG ----
% Mean line
\addplot[
    thick,
    blue,
    mark=none
] table [
    x index=0,
    y index=1,
    col sep=comma
] {conf matrices/learning curves/fed_avg_line.csv};

\addlegendentry{FedAvg}

\addplot[
    thick,
    green,
    mark=none
] table [
    x index=0,
    y index=1,
    col sep=comma
] {conf matrices/learning curves/single_line.csv};
\addlegendentry{Single}

\addplot[
    thick,
    pink,
    mark=none
] table [
    x index=0,
    y index=1,
    col sep=comma
] {conf matrices/learning curves/global_line.csv};

\addlegendentry{Global}

\addplot[
    thick,
    orange,
    mark=none
] table [
    x index=0,
    y index=1,
    col sep=comma
] {conf matrices/learning curves/fed_line_mu_0.csv};
\addlegendentry{\algo, $\lambda=0$}


\addplot[
    thick,
    purple,
    mark=none
] table [
    x index=0,
    y index=1,
    col sep=comma
] {conf matrices/learning curves/fed_line_mu_1000000.csv};
\addlegendentry{\algo, $\lambda=10^6$}

% Confidence interval bounds
\addplot[
    name path=upper,
    draw=none, 
] table [
    x index=0,
    y index=2,
    col sep=comma
] {conf matrices/learning curves/fed_avg_line.csv};

\addplot[
    name path=lower,
    draw=none
] table [
    x index=0,
    y index=3,
    col sep=comma
] {conf matrices/learning curves/fed_avg_line.csv};

% Shaded confidence interval
\addplot[
    blue!20
] fill between[
    of=upper and lower
];





%----- SINGLE ----
% Mean line

% Confidence interval bounds
\addplot[
    name path=upper,
    draw=none
] table [
    x index=0,
    y index=2,
    col sep=comma
] {conf matrices/learning curves/single_line.csv};

\addplot[
    name path=lower,
    draw=none
] table [
    x index=0,
    y index=3,
    col sep=comma
] {conf matrices/learning curves/single_line.csv};

% Shaded confidence interval
\addplot[
    green!20
] fill between[
    of=upper and lower
];



%----- GLOBAL ----
% Mean line

% Confidence interval bounds
\addplot[
    name path=upper,
    draw=none
] table [
    x index=0,
    y index=2,
    col sep=comma
] {conf matrices/learning curves/global_line.csv};

\addplot[
    name path=lower,
    draw=none
] table [
    x index=0,
    y index=3,
    col sep=comma
] {conf matrices/learning curves/global_line.csv};

% Shaded confidence interval
\addplot[
    pink!20
] fill between[
    of=upper and lower
];





%----- FedLoss mu 100 ----
% Mean line


% Confidence interval bounds
\addplot[
    name path=upper,
    draw=none
] table [
    x index=0,
    y index=2,
    col sep=comma
] {conf matrices/learning curves/fed_line_mu_0.csv};

\addplot[
    name path=lower,
    draw=none
] table [
    x index=0,
    y index=3,
    col sep=comma
] {conf matrices/learning curves/fed_line_mu_0.csv};

% Shaded confidence interval
\addplot[
    orange!20
] fill between[
    of=upper and lower
];

%----- FedLoss mu 1000000----
% Mean line


% Confidence interval bounds
\addplot[
    name path=upper,
    draw=none
] table [
    x index=0,
    y index=2,
    col sep=comma
] {conf matrices/learning curves/fed_line_mu_1000000.csv};

\addplot[
    name path=lower,
    draw=none
] table [
    x index=0,
    y index=3,
    col sep=comma
] {conf matrices/learning curves/fed_line_mu_1000000.csv};

% Shaded confidence interval
\addplot[
    purple!20
] fill between[
    of=upper and lower
];
\end{axis}
\end{tikzpicture}

==> review_r1.tex <==
\newcounter{rcnt}
\newcounter{ccnt}

\newcommand{\newreviewernopagebreak}[1]{\vspace{5em} \setcounter{ccnt}{0}\section*{\normalsize Comments of #1}\vspace{4mm}}

\newcommand{\ThisIsTheEditor}{%\clearpage%
\vspace{-5em}\ThisIsTheEditorNoPageBreak}
\newcommand{\ThisIsTheEditorNoPageBreak}{\setcounter{ccnt}{0}\section*{\Large Comments of the Editor}\vspace{3mm}}
\newcommand{\ThisIsANewReviewerNoPageBreak}[1]{\vspace{5em} \refstepcounter{rcnt}\label{r#1}\setcounter{ccnt}{0}\section*{\Large Comments of Reviewer #1}\vspace{3mm}}
\newcommand{\ThisIsANewReviewer}[1]{%\clearpage
\vspace{-5em} \ThisIsANewReviewerNoPageBreak{#1}}


\newcommand{\edcomment}[1]{\fontsize{12}{15}\selectfont
\refstepcounter{ccnt}\label{e\arabic{ccnt}}\noindent\textbf{\boldmath\emph{Comment E.\arabic{ccnt}:} #1}\vspace{0.2cm}}
\newcommand{\refedcomment}[1]{E.\ref{e#1}}

\newcommand{\revcomment}[1]{\refstepcounter{ccnt}\label{r\arabic{rcnt}c\arabic{ccnt}}{\noindent\textbf{\boldmath\emph{Comment \arabic{rcnt}.\arabic{ccnt}:} #1}}\vspace{0.2cm}}
\newcommand{\refrevcomment}[2]{\ref{r#1}.\ref{r#1c#2}}

% \newcommand{\ouranswer}[1]{\noindent\emph{Answer:} #1\vspace{0.6cm}}
% \newcommand{\citepap}[1]{\vspace{0.33cm}\begin{minipage}{0.05\textwidth} $\phantom{A}$  \end{minipage}\begin{minipage}{0.85\textwidth}\renewcommand{\baselinestretch}{1.15}\small \emph{#1} \end{minipage}\vspace{0.3cm}}


\newlength{\ansspace}
\addtolength{\ansspace}{0.6cm}
\newcommand{\ansbreak}{\vspace{\ansspace}}

\newlength{\stdleftskip}
\addtolength{\stdleftskip}{\leftskip}
\newlength{\stdrightskip}
\addtolength{\stdrightskip}{\rightskip}
\newlength{\citeskip}
\addtolength{\citeskip}{3em}
\newcommand{\oldbaselinestretch}{1.25}

\newcommand{\setcitepapskip}{%
    \leftskip\citeskip %
    \rightskip\citeskip %
    \renewcommand{\baselinestretch}{1.15}\small%
    \vspace{0.6em}%
    \noindent%
    \fontsize{10}{12.5}\selectfont
}

\newcommand{\resetLRmargins}{%
    \leftskip\stdleftskip %
    \rightskip\stdrightskip %
    \renewcommand{\baselinestretch}{\oldbaselinestretch}\normalsize %
    \vspace{0.6em}
    \fontsize{12}{15}\selectfont
}

\newcommand{\emans}{\fontsize{12}{15}\selectfont\emph{Answer:\ }}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \setcounter{page}{1}
% \renewcommand{\thepage}{RL -- jmse-1713325 -- Page~\arabic{page}}

\noindent
\begin{minipage}{\linewidth}
\centering
 \vspace{5mm}
 {\huge    Response to Reviewers for manuscript\\[2mm] IoT-67790-2026} \\[5mm]
 {\LARGE ``FedSwitch: Federated Region Classification From Channel Measurements in Vehicular IoT Networks''} 
\end{minipage}

\vspace{5mm}
\noindent
\begin{minipage}{\linewidth}
    \centering   
    {\large Mattia~Piana, Stefano~Rini, and Stefano~Tomasin}
\end{minipage}

\renewcommand{\baselinestretch}{\oldbaselinestretch}\normalsize

\vspace{10mm}


 \section*{\Large Summary of changes}
 \vspace{1mm}
 \fontsize{12}{14}\selectfont
 
\hl{TBD}
 \vspace{4mm}

 \hspace{4cm}Kind regards,

 \vspace{4mm}

 {\hspace{10cm} \large \textit{The Authors}}

\clearpage



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%                     R E V I E W E R   1,2,3                    %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage

\ThisIsANewReviewer{1}
\emph{Comment 1.1}: \textbf{The practical necessity of the considered channel-based region verification task should be better justified. Since base-station locations and coverage areas are generally known, checking whether the vehicle is connected to a base station covering its claimed region may already provide a basic correspondence between vehicle identity and location. CSI may enable finer-grained spatial verification, but the manuscript should explain which applications require this additional accuracy.}


\emans  We thank the reviewer for this comment. We have added the following sentence in the Introduction:

\recalltext{rev1.1} 

\hl{Si potrebbe aggiungere un ulteriore commento all'inizio della sezione numerical results. Ma visto che la spaziatura media tra le BS è 500 metri e le nostre regioni sono di 400 m anche, siamo sicuri che non domini la BS più vicina nella decisione? Sarebbe quasi da simulare una classificazione basata solo sulla copertura delle bs...}

\emph{Comment 1.2}: \textbf{ The motivation and novelty of this paper are not clear. The related-work section largely lists existing studies without carefully explaining their differences from this work. Moreover, collaborative pretraining followed by local fine-tuning is already a widely used personalization strategy in federated learning. The authors should clarify the fundamental distinction between FedSwitch and existing personalized or multi-stage FL methods and identify the technical challenge that is unique to channel-based region classification.}


\emans  \hl{TBD: tutti}

\emph{Comment 1.3}: \textbf{Base-station density and spatial deployment can differ substantially across regions. Consequently, channel measurements collected in one area may not be representative of those observed in another area. The manuscript should analyze how FedSwitch behaves under nonuniform BS density and irregular BS placement. Such analysis is important for understanding whether the method can be transferred to a new geographical deployment.}

\emans  \recalltext{rev1.3}


\emph{Comment 1.4}: \textbf{ The channel model does not account for co-channel interference. Such interference is neither negligible nor stationary and may be difficult to predict. Since the classifier treats CSI variations as location-dependent fingerprints, interference-induced variations may be incorrectly interpreted as changes in the transmitter’s region. The proposed method should therefore be evaluated under different interference levels.
}

\emans  \hl{QUI DIREI CHE IL FOCUS SI é ORA SPOSTATO SU RETI CELLULARI, DOVE L'INTERFERENZA è LIMITATA BY DESIGN E TIPICAMENTE CONSIDERATA TRASCURABILE}

\emph{Comment 1.5}: \textbf{High vehicle mobility means that the region classification decision must be made in real time and may become outdated quickly. The authors should report the inference latency and investigate whether the system can continuously classify numerous vehicles over a long operating period.}

\emans  Questo commento cade perchè non siamo più in high mobility.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%                     R E V I E W E R 2                     %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\ThisIsANewReviewer{2}


\emph{Comment 2.1}: \textbf{ The novelty of FedSwitch with respect to existing personalized and multi-stage federated learning methods should be further clarified. As already discussed in the related-work section, collaborative pre-training followed by client-specific fine-tuning is a well-established strategy. Therefore, the main novelty appears to lie in the adaptive switching criterion. The authors are strongly recommended to compare FedSwitch with representative personalized FL approaches and, more importantly, with a simple FedAvg + fixed-round local fine-tuning baseline to demonstrate the actual benefit brought by the proposed adaptive switching mechanism.}


\emans  \recalltext{rev2.1}

\emph{Comment 2.2}: \textbf{ The switching condition in (16) appears to require careful examination. The manuscript defines the average loss improvement using ($F_k(w_k^{(e)})-F_k(w_k^{(e-1)})$) and triggers personalization when this quantity is smaller than a positive tolerance ($\epsilon$). However, when the training loss is normally decreasing, this difference is negative and therefore already smaller than any positive ($\epsilon$), which seems inconsistent with the intended “loss stagnation” interpretation. Please check the sign and definition of the switching criterion and its implementation in Algorithm 1 carefully.}


\emans  \recalltext{rev2.2.1}



\emph{Comment 2.3}: \textbf{The proposed switching strategy also raises a synchronization issue. Although each BS is independently marked as ready for personalization, no BS actually enters the fine-tuning phase until all BSs satisfy the switching condition. Therefore, the global switching time is effectively determined by the slowest BS, which may introduce unnecessary communication rounds under highly heterogeneous conditions. The authors should discuss this issue and compare the current synchronized switching scheme with client-specific asynchronous switching. Sensitivity analyses with respect to ($T_W$), ($\epsilon$), and the schedule of ($\alpha_t$) are also necessary.}

\emans  \recalltext{rev2.3}

Non ho fatto sensitivity analisis, non c'è spazio


\emph{Comment 2.4}: \textbf{The applicability of Theorem 5.1 to the implemented learning system should be clarified. The theoretical analysis assumes a smooth and strongly convex loss, whereas the numerical experiments employ a ResNet-18 neural network with a multi-class cross-entropy objective, which is clearly non-convex. Moreover, Theorem 5.1 analyzes the optimality gap in (28), which is only introduced as a proxy for the actual windowed switching criterion in (16). Therefore, the current statement that the theorem guarantees the practical switching behavior appears stronger than what is directly established. The authors should clearly distinguish the theoretical setting from the deep-learning implementation and moderate the corresponding claims.
}

\emans  \hl{TBD: SR}

\emph{Comment 2.5}: \textbf{A similar concern exists for Theorem 5.2. The analysis is restricted to a binary CRC problem with (K=2) BSs and (N=2) regions and compares the Neyman–Pearson test obtained from local distributions with that obtained from pooled distributions. However, the actual FedSwitch experiments consider a multi-class neural classifier with (K=5) and (N=7). Thus, the theorem mainly demonstrates the potential disadvantage of global aggregation under distribution mismatch rather than directly establishing a performance guarantee for FedSwitch itself. The scope and implication of this theoretical result should be stated more precisely.}

\emans  \hl{TBD: SR}


\emph{Comment 2.6}: \textbf{The privacy claims should be reconsidered. The manuscript repeatedly states that FedSwitch preserves edge-level privacy because raw CSI measurements are not transmitted to the parameter server. However, standard federated learning does not by itself guarantee privacy, since shared model updates may leak information about local training data. Unless differential privacy, secure aggregation, or another explicit privacy mechanism is incorporated and analyzed, the authors should avoid claiming privacy preservation and instead state more precisely that raw channel measurements remain local.}

\emans We thank the reviewer for this observation. With reference to privacy we wanted to highlight one of the major advantages of federated learning approaches, although we agree that further security mechanisms should be implemented. Since, howeve,r this is not the main focus of the paper, we prefer to reduce and refined references to privacy in the revised manuscript. In particular:
\begin{itemize}
\item we have removed reference to privacy in the abstract,
\item we have modified a paragraph in Introduction as follows: \recalltext{rev2.6}
\end{itemize}
\emph{Comment 2.7}: \textbf{The experimental baseline set is insufficient for evaluating the main contribution. The current comparisons are limited to Global, Single, FedAvg, and FedProx, while FedSwitch is explicitly proposed as a personalized FL method. Comparisons with representative personalized FL methods, as well as other two-stage or local-adaptation strategies, are therefore necessary. Otherwise, the current results mainly demonstrate that personalization can outperform a single global model under non-IID data, rather than that the particular FedSwitch design is superior.}

\emans  \recalltext{rev2.1} \\

and \\

\recalltext{rev2.7} 


\emph{Comment 2.8}: \textbf{The numerical evaluation is entirely based on synthetically generated channel measurements. Although the adopted channel model follows 3GPP specifications, the practical robustness of CSI-based region classification may be significantly affected by mobility, temporal channel variation, environment mismatch, blockage, and changes in propagation conditions. The authors are encouraged to provide validation using measured channel data or, at minimum, introduce more realistic distribution shifts and dynamic vehicular scenarios to evaluate whether the learned region fingerprints remain reliable beyond the assumed simulation model.}

\emans  We thank the reviewer for this suggestion. However, reference datasets are unavailable for the scenario in which the full CSI is used rather than the RSSI alone. Conducting an experimental campaign is beyond the scope of this work. Lastly, we note that the 3GPP channel model captures all the listed phenomena and has been adopted by the standards community to provide a common, realistic scenario for comparing different communication solutions. Thus, we consider the results obtained by simulating it to be very reliable for a scientific paper, while leaving further investigation to industrial projects oriented toward designing a specific product. 


%\setcitepapskip

%\recalltext{rev 4 final}

\resetLRmargins 
